Analysis of Fleet Management and Network Design for On-Demand Urban Air Mobility Operations

A significant challenge in estimating operational feasibility of Urban Air Mobility (UAM) missions lies in understanding how choices in design impact the performance of a complex system-of-systems. This work examines the ability of the UAM ecosystem and the operations within it to meet a variety of demand profiles that may emerge in the coming years. We perform a set of simulation driven feasibility and scalability analyses based on UAM operational models with the goal of estimating capacity and throughput for a given set of parameters that represent an operational UAM ecosystem. UAM ecosystem design guidelines, vehicle constraints, and effective operational policies can be drawn from our analysis. Results show that, while critical for enabling UAM, the performance of the UAM ecosystem is robust to variations in ground infrastructure and fleet design decisions, while being sensitive to decisions for fleet and traffic management policies. We show that so long as the ecosystem design parameters for ground infrastructure and fleet design fall within a sensible range, the performance of the UAM ecosystem is affected by the policies used to manage the UAM traffic.

==> abstract_figs/full_util_demands/t_pax_22.tex <==
% This file was created by tikzplotlib v0.8.5.
\begin{tikzpicture}

\begin{axis}[
colorbar,
% colorbar style={ylabel={Total Hourly Demand}},
colormap/viridis,
point meta max=226.666666666667,
point meta min=2.30769230769231,
tick align=outside,
tick pos=left,
title={Contours of $\hat{d}_\mathrm{max}$ given average \(\displaystyle \Delta t_\text{passenger, min}\) $\approx$ 22 min},
x grid style={white!69.01960784313725!black},
xlabel={Fleet Size, \(\displaystyle f\)},
xmin=-0.5, xmax=100.6,
xtick style={color=black},
xtick={0,18,38,58,78,98},
xticklabels={2,20,40,60,80,100},
y dir=reverse,
y grid style={white!69.01960784313725!black},
ylabel={Avg. Turnaround Time, \(\displaystyle \Delta t_\mathrm{turnaround}\) (min)},
ymin=-0.5, ymax=25.5,
ytick style={color=black},
ytick={0,5,10,15,20,25},
yticklabels={30,25,20,15,10,5},
width={4in}, height={2.7in},
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=100.5, ymin=25.5, ymax=-0.5] {abstract_figs/full_util_demands/t_pax_22-000.png};
\addplot [draw=none]
table{%
x                      y
-3.33066907387547e-17 -0.707106781186547
0.424264068711928 0
2.22044604925031e-17 0.707106781186547
-0.424264068711929 1.11022302462516e-16
-3.33066907387547e-17 -0.707106781186547
};
\path [draw=red, semithick]
(axis cs:2.5,25)
--(axis cs:2.66666666666667,24)
--(axis cs:2.83333333333333,23)
--(axis cs:3,22)
--(axis cs:3.16666666666667,21)
--(axis cs:3.33333333333333,20)
--(axis cs:3.5,19)
--(axis cs:3.64618930710619,18.1228641573629);

\path [draw=red, semithick]
(axis cs:4.02047735956048,15.8771358426371)
--(axis cs:4.16666666666667,15)
--(axis cs:4.33333333333333,14)
--(axis cs:4.5,13)
--(axis cs:4.66666666666667,12)
--(axis cs:4.83333333333333,11)
--(axis cs:5,10)
--(axis cs:5.16666666666667,9)
--(axis cs:5.33333333333333,8)
--(axis cs:5.5,7)
--(axis cs:5.66666666666667,6)
--(axis cs:5.83333333333333,5)
--(axis cs:6,4)
--(axis cs:6.16666666666667,3)
--(axis cs:6.33333333333333,2)
--(axis cs:6.5,1)
--(axis cs:6.66666666666667,0);

\path [draw=red, semithick]
(axis cs:7,25)
--(axis cs:7.33333333333333,24)
--(axis cs:7.66666666666667,23)
--(axis cs:8,22)
--(axis cs:8.33333333333333,21)
--(axis cs:8.66666666666667,20)
--(axis cs:9,19)
--(axis cs:9.29501785942853,18.1149464217144);

\path [draw=red, semithick]
(axis cs:10.0383154739048,15.8850535782856)
--(axis cs:10.3333333333333,15)
--(axis cs:10.6666666666667,14)
--(axis cs:11,13)
--(axis cs:11.3333333333333,12)
--(axis cs:11.6666666666667,11)
--(axis cs:12,10)
--(axis cs:12.3333333333333,9)
--(axis cs:12.6666666666667,8)
--(axis cs:13,7)
--(axis cs:13.3333333333333,6)
--(axis cs:13.6666666666667,5)
--(axis cs:14,4)
--(axis cs:14.3333333333333,3)
--(axis cs:14.6666666666667,2)
--(axis cs:15,1)
--(axis cs:15.3333333333333,0);

\path [draw=red, semithick]
(axis cs:16,25)
--(axis cs:16.6666666666667,24)
--(axis cs:17,23.4912280701754)
--(axis cs:17.3333333333333,23)
--(axis cs:18,22)
--(axis cs:18.6666666666667,21)
--(axis cs:19,20.4920634920635)
--(axis cs:19.3333333333333,20)
--(axis cs:20,19)
--(axis cs:20.6666666666667,18)
--(axis cs:21,17.4927536231884)
--(axis cs:21.3333333333333,17)
--(axis cs:22,16)
--(axis cs:22.6666666666667,15)
--(axis cs:23,14.4933333333333)
--(axis cs:23.3333333333333,14)
--(axis cs:24,13)
--(axis cs:24.6666666666667,12)
--(axis cs:25,11.4938271604938)
--(axis cs:25.3333333333333,11)
--(axis cs:26,10)
--(axis cs:26.6666666666667,9)
--(axis cs:27,8.49425287356322)
--(axis cs:27.2761416459006,8.08480146757264);

\path [draw=red, semithick]
(axis cs:28.7226880315549,5.9150643822662)
--(axis cs:29,5.49462365591398)
--(axis cs:29.3333333333333,5)
--(axis cs:30,4)
--(axis cs:30.6666666666667,3)
--(axis cs:31,2.49494949494949)
--(axis cs:31.3333333333333,2)
--(axis cs:32,1)
--(axis cs:32.6666666666667,0);

\path [draw=red, semithick]
(axis cs:25,25)
--(axis cs:26,24)
--(axis cs:27,23)
--(axis cs:28,22)
--(axis cs:29,21)
--(axis cs:30,20)
--(axis cs:31,19)
--(axis cs:31.9602614214842,18.0397385785158);

\path [draw=red, semithick]
(axis cs:34.0397385785158,15.9602614214842)
--(axis cs:35,15)
--(axis cs:36,14)
--(axis cs:37,13)
--(axis cs:38,12)
--(axis cs:39,11)
--(axis cs:40,10)
--(axis cs:41,9)
--(axis cs:42,8)
--(axis cs:43,7)
--(axis cs:44,6)
--(axis cs:45,5)
--(axis cs:46,4)
--(axis cs:47,3)
--(axis cs:48,2)
--(axis cs:49,1)
--(axis cs:50,0);

\path [draw=red, semithick]
(axis cs:34,25)
--(axis cs:35,24.2432432432432)
--(axis cs:35.3333333333333,24)
--(axis cs:36,23.4912280701754)
--(axis cs:36.6666666666667,23)
--(axis cs:37,22.7435897435897)
--(axis cs:38,22)
--(axis cs:39,21.2439024390244)
--(axis cs:39.3333333333333,21)
--(axis cs:40,20.4920634920635)
--(axis cs:40.6666666666667,20)
--(axis cs:41,19.7441860465116)
--(axis cs:42,19)
--(axis cs:43,18.2444444444444)
--(axis cs:43.3333333333333,18)
--(axis cs:44,17.4927536231884)
--(axis cs:44.6666666666667,17)
--(axis cs:45,16.7446808510638)
--(axis cs:46,16)
--(axis cs:47,15.2448979591837)
--(axis cs:47.3333333333333,15)
--(axis cs:48,14.4933333333333)
--(axis cs:48.6666666666667,14)
--(axis cs:49,13.7450980392157)
--(axis cs:50,13)
--(axis cs:51,12.2452830188679)
--(axis cs:51.3333333333333,12)
--(axis cs:52,11.4938271604938)
--(axis cs:52.6666666666667,11)
--(axis cs:53,10.7454545454545)
--(axis cs:54,10)
--(axis cs:55,9.24561403508772)
--(axis cs:55.3333333333333,9)
--(axis cs:56,8.49425287356322)
--(axis cs:56.6666666666667,8)
--(axis cs:57,7.74576271186441)
--(axis cs:58,7)
--(axis cs:59,6.24590163934426)
--(axis cs:59.3333333333333,6)
--(axis cs:59.3530846528166,5.98502722555298);

\path [draw=red, semithick]
(axis cs:61.9800086911826,4.01491415102254)
--(axis cs:62,4)
--(axis cs:63,3.24615384615385)
--(axis cs:63.3333333333333,3)
--(axis cs:64,2.49494949494949)
--(axis cs:64.6666666666667,2)
--(axis cs:65,1.74626865671641)
--(axis cs:66,1)
--(axis cs:67,0.246376811594205)
--(axis cs:67.3333333333333,0);

\path [draw=red, semithick]
(axis cs:43,25)
--(axis cs:44,24.3913043478261)
--(axis cs:44.6666666666667,24)
--(axis cs:45,23.7943262411348)
--(axis cs:46,23.1944444444444)
--(axis cs:46.3333333333333,23)
--(axis cs:47,22.5918367346939)
--(axis cs:48,22)
--(axis cs:49,21.3921568627451)
--(axis cs:49.6666666666667,21)
--(axis cs:50,20.7948717948718)
--(axis cs:51,20.1949685534591)
--(axis cs:51.3333333333333,20)
--(axis cs:52,19.5925925925926)
--(axis cs:53,19)
--(axis cs:54,18.3928571428571)
--(axis cs:54.6666666666667,18)
--(axis cs:55,17.7953216374269)
--(axis cs:56,17.1954022988506)
--(axis cs:56.3333333333333,17)
--(axis cs:57,16.5932203389831)
--(axis cs:58,16)
--(axis cs:59,15.3934426229508)
--(axis cs:59.6666666666667,15)
--(axis cs:60,14.7956989247312)
--(axis cs:61,14.1957671957672)
--(axis cs:61.3333333333333,14)
--(axis cs:62,13.59375)
--(axis cs:63,13)
--(axis cs:64,12.3939393939394)
--(axis cs:64.6666666666667,12)
--(axis cs:65,11.7960199004975)
--(axis cs:66,11.1960784313725)
--(axis cs:66.3333333333333,11)
--(axis cs:67,10.5942028985507)
--(axis cs:67.6386860473541,10.214693797949);

\path [draw=red, semithick]
(axis cs:71.6890270312762,7.78369977827796)
--(axis cs:72,7.59459459459459)
--(axis cs:73,7)
--(axis cs:74,6.39473684210526)
--(axis cs:74.6666666666667,6)
--(axis cs:75,5.7965367965368)
--(axis cs:76,5.19658119658119)
--(axis cs:76.3333333333333,5)
--(axis cs:77,4.59493670886076)
--(axis cs:78,4)
--(axis cs:79,3.39506172839506)
--(axis cs:79.6666666666667,3)
--(axis cs:80,2.79674796747967)
--(axis cs:81,2.19678714859438)
--(axis cs:81.3333333333333,2)
--(axis cs:82,1.5952380952381)
--(axis cs:83,1)
--(axis cs:84,0.395348837209305)
--(axis cs:84.6666666666667,0);

\path [draw=red, semithick]
(axis cs:65.5,25)
--(axis cs:66,24.7941176470588)
--(axis cs:67,24.3913043478261)
--(axis cs:68,24)
--(axis cs:69,23.5915492957746)
--(axis cs:70,23.1944444444444)
--(axis cs:70.5,23)
--(axis cs:71,22.7945205479452)
--(axis cs:72,22.3918918918919)
--(axis cs:73,22)
--(axis cs:74,21.5921052631579)
--(axis cs:75,21.1948051948052)
--(axis cs:75.5,21)
--(axis cs:76,20.7948717948718)
--(axis cs:77,20.3924050632911)
--(axis cs:78,20)
--(axis cs:79,19.5925925925926)
--(axis cs:80,19.1951219512195)
--(axis cs:80.5,19)
--(axis cs:81,18.7951807228916)
--(axis cs:82,18.3928571428571)
--(axis cs:83,18)
--(axis cs:84,17.593023255814)
--(axis cs:85,17.1954022988506)
--(axis cs:85.5,17)
--(axis cs:86,16.7954545454545)
--(axis cs:87,16.3932584269663)
--(axis cs:88,16)
--(axis cs:89,15.5934065934066)
--(axis cs:90,15.195652173913)
--(axis cs:90.5,15)
--(axis cs:91,14.7956989247312)
--(axis cs:92,14.3936170212766)
--(axis cs:93,14)
--(axis cs:93.4372998614296,13.8223469312942);

\path [draw=red, semithick]
(axis cs:98.5652237901179,11.770552718863)
--(axis cs:99,11.5940594059406)
--(axis cs:100,11.1960784313725);

\path [draw=red, semithick]
(axis cs:88,25)
--(axis cs:89,24.6923076923077)
--(axis cs:90,24.3913043478261)
--(axis cs:91,24.0967741935484)
--(axis cs:91.1171970663976,24.0627492387878);

\path [draw=red, semithick]
(axis cs:96.8848745216589,22.3273411551422)
--(axis cs:97,22.2929292929293)
--(axis cs:98,22)
--(axis cs:99,21.6930693069307)
--(axis cs:100,21.3921568627451);


\addplot+[draw=white, mark size = {3}, white,mark=diamond*,mark options={fill=white}] coordinates {
(34, 20)
};
\node at (axis cs:36,20)[
  scale=0.75,
  anchor=base west,
  text=white,
  rotate=0.0
]{Case Study Point};
\node at (axis cs:3.83333333333333,17)[
  scale=0.7,
  text=white,
  rotate=86.0
]{10};
\node at (axis cs:9.66666666666666,17)[
  scale=0.7,
  text=white,
  rotate=82.1
]{20};
\node at (axis cs:28,7)[
  scale=0.7,
  text=white,
  rotate=74.6
]{40};
\node at (axis cs:33,17)[
  scale=0.7,
  text=white,
  rotate=67.5
]{60};
\node at (axis cs:60.6666666666667,5)[
  scale=0.7,
  text=white,
  rotate=61.0
]{80};
\node at (axis cs:69.6666666666667,9)[
  scale=0.7,
  text=white,
  rotate=55.4
]{100};
\node at (axis cs:96,12.7959183673469)[
  scale=0.7,
  text=white,
  rotate=43.9
]{150};
\node at (axis cs:94,23.1944444444444)[
  scale=0.7,
  text=black,
  rotate=36.0
]{200};

\end{axis}

\node [
    scale=1.0,
    text=black,
    rotate=90.0
]at (10.5, 2.5) {Total Demand per Hour};

\end{tikzpicture}


==> abstract_figs/time_util_bay_airspace_3_normalize=False_turnaround=10_policy=no_g_hold_redundancy=0.4.tex <==
% This file was created by tikzplotlib v0.8.5.
% redundancy = 0.4
\begin{tikzpicture}
\small
\definecolor{color0}{rgb}{0.2298057,0.298717966,0.753683153}
\definecolor{color1}{rgb}{0.554311869913725,0.690097011215686,0.995515548235294}
\definecolor{color2}{rgb}{0.867427635086275,0.864376599772549,0.862602462019608}
\definecolor{color3}{rgb}{0.956653210976471,0.598033822717647,0.477302292352941}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.01960784313725!black},
xlabel={Total Demand per Hour},
xmin=-0.751, xmax=6.751,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={3,9,15,21,30,45,60},
y grid style={white!69.01960784313725!black},
ylabel={Average Time Utilization (min)},
ymin=0, ymax=550,
ytick style={color=black},
width={2.5in}, height={2.5in},
]
\draw[draw=red,fill=color0,line width=0.24pt] (axis cs:0.00999999999999998,0) rectangle (axis cs:0.41,22.299363286008);
\draw[draw=red,fill=color0,line width=0.24pt] (axis cs:1.01,0) rectangle (axis cs:1.41,22.3212062313065);
\draw[draw=red,fill=color0,line width=0.24pt] (axis cs:2.01,0) rectangle (axis cs:2.41,22.1554566281484);
\draw[draw=red,fill=color0,line width=0.24pt] (axis cs:3.01,0) rectangle (axis cs:3.41,22.1846391461088);
\draw[draw=red,fill=color0,line width=0.24pt] (axis cs:4.01,0) rectangle (axis cs:4.41,22.1684180912318);
\draw[draw=red,fill=color0,line width=0.24pt] (axis cs:5.01,0) rectangle (axis cs:5.41,22.0962375676688);
\draw[draw=red,fill=color0,line width=0.24pt] (axis cs:6.01,0) rectangle (axis cs:6.41,22.0980162812671);
\draw[draw=red,fill=color1,line width=0.24pt] (axis cs:0.00999999999999998,22.299363286008) rectangle (axis cs:0.41,32.299363286008);
\draw[draw=red,fill=color1,line width=0.24pt] (axis cs:1.01,22.3212062313065) rectangle (axis cs:1.41,32.3212062313065);
\draw[draw=red,fill=color1,line width=0.24pt] (axis cs:2.01,22.1554566281484) rectangle (axis cs:2.41,32.1554566281484);
\draw[draw=red,fill=color1,line width=0.24pt] (axis cs:3.01,22.1846391461088) rectangle (axis cs:3.41,32.1846391461088);
\draw[draw=red,fill=color1,line width=0.24pt] (axis cs:4.01,22.1684180912318) rectangle (axis cs:4.41,32.1684180912318);
\draw[draw=red,fill=color1,line width=0.24pt] (axis cs:5.01,22.0962375676688) rectangle (axis cs:5.41,32.0962375676688);
\draw[draw=red,fill=color1,line width=0.24pt] (axis cs:6.01,22.0980162812671) rectangle (axis cs:6.41,32.0980162812671);
\draw[draw=red,fill=color2,line width=0.24pt] (axis cs:0.00999999999999998,32.299363286008) rectangle (axis cs:0.41,471.403626855916);
\draw[draw=red,fill=color2,line width=0.24pt] (axis cs:1.01,32.3212062313065) rectangle (axis cs:1.41,180.486324860434);
\draw[draw=red,fill=color2,line width=0.24pt] (axis cs:2.01,32.1554566281484) rectangle (axis cs:2.41,112.11348293657);
\draw[draw=red,fill=color2,line width=0.24pt] (axis cs:3.01,32.1846391461088) rectangle (axis cs:3.41,82.3032627745104);
\draw[draw=red,fill=color2,line width=0.24pt] (axis cs:4.01,32.1684180912318) rectangle (axis cs:4.41,59.123690526807);
\draw[draw=red,fill=color2,line width=0.24pt] (axis cs:5.01,32.0962375676688) rectangle (axis cs:5.41,41.1210362898541);
\draw[draw=red,fill=color2,line width=0.24pt] (axis cs:6.01,32.0980162812671) rectangle (axis cs:6.41,32.8435106268264);
\draw[draw=red,fill=color3,line width=0.24pt] (axis cs:0.00999999999999998,471.403626855916) rectangle (axis cs:0.41,472.26743721164);
\draw[draw=red,fill=color3,line width=0.24pt] (axis cs:1.01,180.486324860434) rectangle (axis cs:1.41,181.462432640345);
\draw[draw=red,fill=color3,line width=0.24pt] (axis cs:2.01,112.11348293657) rectangle (axis cs:2.41,112.874347645677);
\draw[draw=red,fill=color3,line width=0.24pt] (axis cs:3.01,82.3032627745104) rectangle (axis cs:3.41,82.9109560293934);
\draw[draw=red,fill=color3,line width=0.24pt] (axis cs:4.01,59.123690526807) rectangle (axis cs:4.41,59.5503713016219);
\draw[draw=red,fill=color3,line width=0.24pt] (axis cs:5.01,41.1210362898541) rectangle (axis cs:5.41,41.2557707934993);
\draw[draw=red,fill=color3,line width=0.24pt] (axis cs:6.01,32.8435106268264) rectangle (axis cs:6.41,32.8435106268264);
\draw[draw=blue,fill=color0,line width=0.24pt] (axis cs:-0.41,0) rectangle (axis cs:-0.01,27.8363456384664);
\draw[draw=blue,fill=color0,line width=0.24pt] (axis cs:0.59,0) rectangle (axis cs:0.99,31.2543028634158);
\draw[draw=blue,fill=color0,line width=0.24pt] (axis cs:1.59,0) rectangle (axis cs:1.99,30.7049681838254);
\draw[draw=blue,fill=color0,line width=0.24pt] (axis cs:2.59,0) rectangle (axis cs:2.99,27.6056905898231);
\draw[draw=blue,fill=color0,line width=0.24pt] (axis cs:3.59,0) rectangle (axis cs:3.99,24.4358709626247);
\draw[draw=blue,fill=color0,line width=0.24pt] (axis cs:4.59,0) rectangle (axis cs:4.99,22.201266346692);
\draw[draw=blue,fill=color0,line width=0.24pt] (axis cs:5.59,0) rectangle (axis cs:5.99,22.1417442841187);
\draw[draw=blue,fill=color1,line width=0.24pt] (axis cs:-0.41,27.8363456384664) rectangle (axis cs:-0.01,37.8363456384664);
\draw[draw=blue,fill=color1,line width=0.24pt] (axis cs:0.59,31.2543028634158) rectangle (axis cs:0.99,41.2543028634158);
\draw[draw=blue,fill=color1,line width=0.24pt] (axis cs:1.59,30.7049681838254) rectangle (axis cs:1.99,40.7049681838254);
\draw[draw=blue,fill=color1,line width=0.24pt] (axis cs:2.59,27.6056905898231) rectangle (axis cs:2.99,37.6056905898231);
\draw[draw=blue,fill=color1,line width=0.24pt] (axis cs:3.59,24.4358709626247) rectangle (axis cs:3.99,34.4358709626247);
\draw[draw=blue,fill=color1,line width=0.24pt] (axis cs:4.59,22.201266346692) rectangle (axis cs:4.99,32.201266346692);
\draw[draw=blue,fill=color1,line width=0.24pt] (axis cs:5.59,22.1417442841187) rectangle (axis cs:5.99,32.1417442841187);
\draw[draw=blue,fill=color2,line width=0.24pt] (axis cs:-0.41,37.8363456384664) rectangle (axis cs:-0.01,477.396421319756);
\draw[draw=blue,fill=color2,line width=0.24pt] (axis cs:0.59,41.2543028634158) rectangle (axis cs:0.99,189.601691595616);
\draw[draw=blue,fill=color2,line width=0.24pt] (axis cs:1.59,40.7049681838254) rectangle (axis cs:1.99,118.603827527772);
\draw[draw=blue,fill=color2,line width=0.24pt] (axis cs:2.59,37.6056905898231) rectangle (axis cs:2.99,85.986778193007);
\draw[draw=blue,fill=color2,line width=0.24pt] (axis cs:3.59,34.4358709626247) rectangle (axis cs:3.99,61.3793700213554);
\draw[draw=blue,fill=color2,line width=0.24pt] (axis cs:4.59,32.201266346692) rectangle (axis cs:4.99,41.461939753669);
\draw[draw=blue,fill=color2,line width=0.24pt] (axis cs:5.59,32.1417442841187) rectangle (axis cs:5.99,32.9096580569994);
\draw[draw=blue,fill=color3,line width=0.24pt] (axis cs:-0.41,477.396421319756) rectangle (axis cs:-0.01,477.396421319756);
\draw[draw=blue,fill=color3,line width=0.24pt] (axis cs:0.59,189.601691595616) rectangle (axis cs:0.99,189.601691595616);
\draw[draw=blue,fill=color3,line width=0.24pt] (axis cs:1.59,118.603827527772) rectangle (axis cs:1.99,118.603827527772);
\draw[draw=blue,fill=color3,line width=0.24pt] (axis cs:2.59,85.986778193007) rectangle (axis cs:2.99,85.986778193007);
\draw[draw=blue,fill=color3,line width=0.24pt] (axis cs:3.59,61.3793700213554) rectangle (axis cs:3.99,61.3793700213554);
\draw[draw=blue,fill=color3,line width=0.24pt] (axis cs:4.59,41.461939753669) rectangle (axis cs:4.99,41.461939753669);
\draw[draw=blue,fill=color3,line width=0.24pt] (axis cs:5.59,32.9096580569994) rectangle (axis cs:5.99,32.9096580569994);
\end{axis}

\begin{axis}[
axis y line=right,
legend cell align={left},
legend entries={{Passenger},{Turnaround},{Idling},{Re-balancing},{Delay w/ re-balancing},{Delay w/o re-balancing},{Estimated $\hat{d}_\mathrm{max}$}},
legend style={at={(0.18,0.6)}, anchor={south west}, nodes={scale=0.7, transform shape}},
tick align=outside,
% title={bay\_airspace\_3, [10, 10, 10], redundancy = 0.4, turnaround\_time = 10 min, no\_g\_hold},
x grid style={white!69.01960784313725!black},
xmin=-0.751, xmax=6.751,
xtick pos=left,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={,,},
y grid style={white!69.01960784313725!black},
ylabel={Average Demand Delay (min)},
ymin=-2.94079568676041, ymax=64.1253746763472,
ytick pos=right,
ytick style={color=black},
width={2.5in}, height={2.5in},
]

\addlegendimage{only marks,mark=square*,color=color0}
\addlegendimage{only marks,mark=square*,color=color1}
\addlegendimage{only marks,mark=square*,color=color2}
\addlegendimage{only marks,mark=square*,color=color3}
\addlegendimage{mark=diamond*,color=red}
\addlegendimage{mark=diamond*,color=blue}
\addlegendimage{mark=--, dashed, color=black}

\path [draw=red, semithick]
(axis cs:0,0.107666602471755)
--(axis cs:0,0.108423259603821);

\path [draw=red, semithick]
(axis cs:1,0.371065399401683)
--(axis cs:1,0.524695434406811);

\path [draw=red, semithick]
(axis cs:2,1.74194493149653)
--(axis cs:2,2.29912821299968);

\path [draw=red, semithick]
(axis cs:3,4.34739998574956)
--(axis cs:3,5.06178843945053);

\path [draw=red, semithick]
(axis cs:4,7.65237635443541)
--(axis cs:4,8.73277998965058);

\path [draw=red, semithick]
(axis cs:5,18.1181558240983)
--(axis cs:5,19.4387187838209);

\path [draw=red, semithick]
(axis cs:6,58.9377217574117)
--(axis cs:6,60.5896160821206);

\path [draw=blue, semithick]
(axis cs:0,0.114527912365749)
--(axis cs:0,0.123511906236645);

\path [draw=blue, semithick]
(axis cs:1,2.58478991098836)
--(axis cs:1,3.42307411473727);

\path [draw=blue, semithick]
(axis cs:2,8.18349117211214)
--(axis cs:2,9.54825929066889);

\path [draw=blue, semithick]
(axis cs:3,10.6001237720138)
--(axis cs:3,12.1301239456726);

\path [draw=blue, semithick]
(axis cs:4,14.4227338366041)
--(axis cs:4,16.0738291128587);

\path [draw=blue, semithick]
(axis cs:5,20.4082040658643)
--(axis cs:5,22.0242750399651);

\path [draw=blue, semithick]
(axis cs:6,59.2599044958363)
--(axis cs:6,61.076912387115);

\addplot [semithick, red, mark=-, mark size=3, mark options={solid}, only marks]
table {%
0 0.107666602471755
1 0.371065399401683
2 1.74194493149653
3 4.34739998574956
4 7.65237635443541
5 18.1181558240983
6 58.9377217574117
};
% \addlegendentry{Demand delay without rebalancing}
\addplot [semithick, red, mark=-, mark size=3, mark options={solid}, only marks]
table {%
0 0.108423259603821
1 0.524695434406811
2 2.29912821299968
3 5.06178843945053
4 8.73277998965058
5 19.4387187838209
6 60.5896160821206
};
% \addlegendentry{Demand delay without rebalancing}
\addplot [semithick, blue, mark=-, mark size=3, mark options={solid}, only marks]
table {%
0 0.114527912365749
1 2.58478991098836
2 8.18349117211214
3 10.6001237720138
4 14.4227338366041
5 20.4082040658643
6 59.2599044958363
};
% \addlegendentry{Demand delay without rebalancing}
\addplot [semithick, blue, mark=-, mark size=3, mark options={solid}, only marks]
table {%
0 0.123511906236645
1 3.42307411473727
2 9.54825929066889
3 12.1301239456726
4 16.0738291128587
5 22.0242750399651
6 61.076912387115
};
% \addlegendentry{Demand delay without rebalancing}
\addplot [semithick, red, mark=diamond*, mark size=2, mark options={solid}]
table {%
0 0.108044931037788
1 0.447880416904247
2 2.0205365722481
3 4.70459421260004
4 8.192578172043
5 18.7784373039596
6 59.7636689197661
};
% \addlegendentry{Demand delay without rebalancing}
\addplot [semithick, blue, mark=diamond*, mark size=2, mark options={solid}]
table {%
0 0.119019909301197
1 3.00393201286282
2 8.86587523139051
3 11.3651238588432
4 15.2482814747314
5 21.2162395529147
6 60.1684084414757
};
% \addlegendentry{Demand delay without rebalancing}
\addplot [semithick, black, dashed]
table {%
5.73 99
5.73 -10
};
\end{axis}

\end{tikzpicture}


==> abstract_figs/time_util_bay_airspace_3_normalize=False_turnaround=10_policy=no_g_hold_redundancy=0.tex <==
% This file was created by tikzplotlib v0.8.5.
% redundancy = 0
\begin{tikzpicture}
\small
\definecolor{color0}{rgb}{0.2298057,0.298717966,0.753683153}
\definecolor{color1}{rgb}{0.554311869913725,0.690097011215686,0.995515548235294}
\definecolor{color2}{rgb}{0.867427635086275,0.864376599772549,0.862602462019608}
\definecolor{color3}{rgb}{0.956653210976471,0.598033822717647,0.477302292352941}

% \begin{groupplot}[group style={vertical sep = 1.3cm, group size=1 by 2}]
% \nextgroupplot
\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.01960784313725!black},
xlabel={Total Demand per Hour},
xmin=-0.751, xmax=6.751,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={3,9,15,21,30,45,60},
y grid style={white!69.01960784313725!black},
ylabel={Average Time Utilization (min)},
ymin=0, ymax=550,
ytick style={color=black},
width={2.5in}, height={2.5in},
]
\node[style=rectangle, draw=blue] at (320, 450) {Without re-balancing};
\node[style=rectangle, draw=red] at (330, 300) {With re-balancing};

\draw[draw=red,fill=color0,line width=0.24pt] (axis cs:0.00999999999999998,0) rectangle (axis cs:0.41,23.8330518355131);
\draw[draw=red,fill=color0,line width=0.24pt] (axis cs:1.01,0) rectangle (axis cs:1.41,22.9165390408336);
\draw[draw=red,fill=color0,line width=0.24pt] (axis cs:2.01,0) rectangle (axis cs:2.41,22.5853199408311);
\draw[draw=red,fill=color0,line width=0.24pt] (axis cs:3.01,0) rectangle (axis cs:3.41,22.4843484642545);
\draw[draw=red,fill=color0,line width=0.24pt] (axis cs:4.01,0) rectangle (axis cs:4.41,22.3631169842233);
\draw[draw=red,fill=color0,line width=0.24pt] (axis cs:5.01,0) rectangle (axis cs:5.41,22.1549082494033);
\draw[draw=red,fill=color0,line width=0.24pt] (axis cs:6.01,0) rectangle (axis cs:6.41,22.1145802518574);
\draw[draw=red,fill=color1,line width=0.24pt] (axis cs:0.00999999999999998,23.8330518355131) rectangle (axis cs:0.41,33.8330518355131);
\draw[draw=red,fill=color1,line width=0.24pt] (axis cs:1.01,22.9165390408336) rectangle (axis cs:1.41,32.9165390408336);
\draw[draw=red,fill=color1,line width=0.24pt] (axis cs:2.01,22.5853199408311) rectangle (axis cs:2.41,32.5853199408311);
\draw[draw=red,fill=color1,line width=0.24pt] (axis cs:3.01,22.4843484642545) rectangle (axis cs:3.41,32.4843484642545);
\draw[draw=red,fill=color1,line width=0.24pt] (axis cs:4.01,22.3631169842233) rectangle (axis cs:4.41,32.3631169842233);
\draw[draw=red,fill=color1,line width=0.24pt] (axis cs:5.01,22.1549082494033) rectangle (axis cs:5.41,32.1549082494033);
\draw[draw=red,fill=color1,line width=0.24pt] (axis cs:6.01,22.1145802518574) rectangle (axis cs:6.41,32.1145802518574);
\draw[draw=red,fill=color2,line width=0.24pt] (axis cs:0.00999999999999998,33.8330518355131) rectangle (axis cs:0.41,323.684642344454);
\draw[draw=red,fill=color2,line width=0.24pt] (axis cs:1.01,32.9165390408336) rectangle (axis cs:1.41,144.522049597934);
\draw[draw=red,fill=color2,line width=0.24pt] (axis cs:2.01,32.5853199408311) rectangle (axis cs:2.41,95.7950823705865);
\draw[draw=red,fill=color2,line width=0.24pt] (axis cs:3.01,32.4843484642545) rectangle (axis cs:3.41,73.2474672504401);
\draw[draw=red,fill=color2,line width=0.24pt] (axis cs:4.01,32.3631169842233) rectangle (axis cs:4.41,53.7726247764154);
\draw[draw=red,fill=color2,line width=0.24pt] (axis cs:5.01,32.1549082494033) rectangle (axis cs:5.41,39.1615583769244);
\draw[draw=red,fill=color2,line width=0.24pt] (axis cs:6.01,32.1145802518574) rectangle (axis cs:6.41,32.8258071134613);
\draw[draw=red,fill=color3,line width=0.24pt] (axis cs:0.00999999999999998,323.684642344454) rectangle (axis cs:0.41,337.272408687462);
\draw[draw=red,fill=color3,line width=0.24pt] (axis cs:1.01,144.522049597934) rectangle (axis cs:1.41,150.976729051103);
\draw[draw=red,fill=color3,line width=0.24pt] (axis cs:2.01,95.7950823705865) rectangle (axis cs:2.41,100.197145879935);
\draw[draw=red,fill=color3,line width=0.24pt] (axis cs:3.01,73.2474672504401) rectangle (axis cs:3.41,76.4296813205579);
\draw[draw=red,fill=color3,line width=0.24pt] (axis cs:4.01,53.7726247764154) rectangle (axis cs:4.41,55.9862910735773);
\draw[draw=red,fill=color3,line width=0.24pt] (axis cs:5.01,39.1615583769244) rectangle (axis cs:5.41,39.9251329009245);
\draw[draw=red,fill=color3,line width=0.24pt] (axis cs:6.01,32.8258071134613) rectangle (axis cs:6.41,32.8592068522341);
\draw[draw=blue,fill=color0,line width=0.24pt] (axis cs:-0.41,0) rectangle (axis cs:-0.01,80.5908255666526);
\draw[draw=blue,fill=color0,line width=0.24pt] (axis cs:0.59,0) rectangle (axis cs:0.99,52.9918287771157);
\draw[draw=blue,fill=color0,line width=0.24pt] (axis cs:1.59,0) rectangle (axis cs:1.99,41.3377532511743);
\draw[draw=blue,fill=color0,line width=0.24pt] (axis cs:2.59,0) rectangle (axis cs:2.99,35.0809529121051);
\draw[draw=blue,fill=color0,line width=0.24pt] (axis cs:3.59,0) rectangle (axis cs:3.99,29.1639760858316);
\draw[draw=blue,fill=color0,line width=0.24pt] (axis cs:4.59,0) rectangle (axis cs:4.99,23.540929031054);
\draw[draw=blue,fill=color0,line width=0.24pt] (axis cs:5.59,0) rectangle (axis cs:5.99,22.1506325459185);
\draw[draw=blue,fill=color1,line width=0.24pt] (axis cs:-0.41,80.5908255666526) rectangle (axis cs:-0.01,90.5908255666526);
\draw[draw=blue,fill=color1,line width=0.24pt] (axis cs:0.59,52.9918287771157) rectangle (axis cs:0.99,62.9918287771157);
\draw[draw=blue,fill=color1,line width=0.24pt] (axis cs:1.59,41.3377532511743) rectangle (axis cs:1.99,51.3377532511743);
\draw[draw=blue,fill=color1,line width=0.24pt] (axis cs:2.59,35.0809529121051) rectangle (axis cs:2.99,45.0809529121051);
\draw[draw=blue,fill=color1,line width=0.24pt] (axis cs:3.59,29.1639760858316) rectangle (axis cs:3.99,39.1639760858316);
\draw[draw=blue,fill=color1,line width=0.24pt] (axis cs:4.59,23.540929031054) rectangle (axis cs:4.99,33.540929031054);
\draw[draw=blue,fill=color1,line width=0.24pt] (axis cs:5.59,22.1506325459185) rectangle (axis cs:5.99,32.1506325459185);
\draw[draw=blue,fill=color2,line width=0.24pt] (axis cs:-0.41,90.5908255666526) rectangle (axis cs:-0.01,507.892472381184);
\draw[draw=blue,fill=color2,line width=0.24pt] (axis cs:0.59,62.9918287771157) rectangle (axis cs:0.99,194.652975346894);
\draw[draw=blue,fill=color2,line width=0.24pt] (axis cs:1.59,51.3377532511743) rectangle (axis cs:1.99,120.321758533847);
\draw[draw=blue,fill=color2,line width=0.24pt] (axis cs:2.59,45.0809529121051) rectangle (axis cs:2.99,86.8344658030227);
\draw[draw=blue,fill=color2,line width=0.24pt] (axis cs:3.59,39.1639760858316) rectangle (axis cs:3.99,61.5003589971675);
\draw[draw=blue,fill=color2,line width=0.24pt] (axis cs:4.59,33.540929031054) rectangle (axis cs:4.99,41.6054986705537);
\draw[draw=blue,fill=color2,line width=0.24pt] (axis cs:5.59,32.1506325459185) rectangle (axis cs:5.99,32.8686519795822);
\draw[draw=blue,fill=color3,line width=0.24pt] (axis cs:-0.41,507.892472381184) rectangle (axis cs:-0.01,507.892472381184);
\draw[draw=blue,fill=color3,line width=0.24pt] (axis cs:0.59,194.652975346894) rectangle (axis cs:0.99,194.652975346894);
\draw[draw=blue,fill=color3,line width=0.24pt] (axis cs:1.59,120.321758533847) rectangle (axis cs:1.99,120.321758533847);
\draw[draw=blue,fill=color3,line width=0.24pt] (axis cs:2.59,86.8344658030227) rectangle (axis cs:2.99,86.8344658030227);
\draw[draw=blue,fill=color3,line width=0.24pt] (axis cs:3.59,61.5003589971675) rectangle (axis cs:3.99,61.5003589971675);
\draw[draw=blue,fill=color3,line width=0.24pt] (axis cs:4.59,41.6054986705537) rectangle (axis cs:4.99,41.6054986705537);
\draw[draw=blue,fill=color3,line width=0.24pt] (axis cs:5.59,32.8686519795822) rectangle (axis cs:5.99,32.8686519795822);
\end{axis}

\begin{axis}[
axis y line=right,
% legend cell align={left},
% legend entries={{Passenger},{Turnaround},{Idling},{Re-balancing},{Delay with re-balancing},{Delay without re-balancing}},
% legend style={at={(1.3,0.2)}, anchor={south west}},
tick align=outside,
% title={bay\_airspace\_3, [10, 10, 10], redundancy = 0, turnaround\_time = 10 min, no\_g\_hold},
x grid style={white!69.01960784313725!black},
xmin=-0.751, xmax=6.751,
xtick pos=left,
xtick style={color=black},
xtick={0,1,2,3,4,5,6},
xticklabels={,,},
y grid style={white!69.01960784313725!black},
ylabel={Average Demand Delay (min)},
ymin=-2.9937041214224, ymax=65.2341681715857,
ytick pos=right,
ytick style={color=black},
width={2.5in}, height={2.5in},
]
% \addlegendimage{only marks,mark=square*,color=color0}
% \addlegendimage{only marks,mark=square*,color=color1}
% \addlegendimage{only marks,mark=square*,color=color2}
% \addlegendimage{only marks,mark=square*,color=color3}
% \addlegendimage{mark=*,color=red}
% \addlegendimage{mark=*,color=blue}

\path [draw=red, semithick]
(axis cs:0,0.107562800987062)
--(axis cs:0,0.108459857961495);

\path [draw=red, semithick]
(axis cs:1,0.107773054250032)
--(axis cs:1,0.108283331055513);

\path [draw=red, semithick]
(axis cs:2,0.109033813089629)
--(axis cs:2,0.109718740289591);

\path [draw=red, semithick]
(axis cs:3,0.153813565032848)
--(axis cs:3,0.165480003504014);

\path [draw=red, semithick]
(axis cs:4,1.01389294507173)
--(axis cs:4,1.14133658318201);

\path [draw=red, semithick]
(axis cs:5,9.23032327361059)
--(axis cs:5,10.0376528413134);

\path [draw=red, semithick]
(axis cs:6,59.7765243077485)
--(axis cs:6,61.300172741411);

\path [draw=blue, semithick]
(axis cs:0,0.108826031754231)
--(axis cs:0,0.122373408841051);

\path [draw=blue, semithick]
(axis cs:1,2.05177852682173)
--(axis cs:1,2.84574009744957);

\path [draw=blue, semithick]
(axis cs:2,5.42345608163086)
--(axis cs:2,6.65848144524828);

\path [draw=blue, semithick]
(axis cs:3,9.25970464176837)
--(axis cs:3,10.8706033529456);

\path [draw=blue, semithick]
(axis cs:4,13.1734425380853)
--(axis cs:4,14.953354090647);

\path [draw=blue, semithick]
(axis cs:5,22.8301397934532)
--(axis cs:5,24.5021915084442);

\path [draw=blue, semithick]
(axis cs:6,60.4390958386423)
--(axis cs:6,62.1329012491762);

\addplot [semithick, red, mark=-, mark size=3, mark options={solid}, only marks]
table {%
0 0.107562800987062
1 0.107773054250032
2 0.109033813089629
3 0.153813565032848
4 1.01389294507173
5 9.23032327361059
6 59.7765243077485
};
% \addlegendentry{Demand delay without rebalancing}
\addplot [semithick, red, mark=-, mark size=3, mark options={solid}, only marks]
table {%
0 0.108459857961495
1 0.108283331055513
2 0.109718740289591
3 0.165480003504014
4 1.14133658318201
5 10.0376528413134
6 61.300172741411
};
% \addlegendentry{Demand delay without rebalancing}
\addplot [semithick, blue, mark=-, mark size=3, mark options={solid}, only marks]
table {%
0 0.108826031754231
1 2.05177852682173
2 5.42345608163086
3 9.25970464176837
4 13.1734425380853
5 22.8301397934532
6 60.4390958386423
};
% \addlegendentry{Demand delay without rebalancing}
\addplot [semithick, blue, mark=-, mark size=3, mark options={solid}, only marks]
table {%
0 0.122373408841051
1 2.84574009744957
2 6.65848144524828
3 10.8706033529456
4 14.953354090647
5 24.5021915084442
6 62.1329012491762
};
% \addlegendentry{Demand delay without rebalancing}
\addplot [semithick, red, mark=diamond*, mark size=2, mark options={solid}]
table {%
0 0.108011329474279
1 0.108028192652772
2 0.10937627668961
3 0.159646784268431
4 1.07761476412687
5 9.63398805746199
6 60.5383485245798
};
% \addlegendentry{Demand delay without rebalancing}
\addplot [semithick, blue, mark=diamond*, mark size=2, mark options={solid}]
table {%
0 0.115599720297641
1 2.44875931213565
2 6.04096876343957
3 10.065153997357
4 14.0633983143662
5 23.6661656509487
6 61.2859985439093
};
% \addlegendentry{Demand delay without rebalancing}
\addplot [semithick, black, dashed]
table {%
5.73 99
5.73 -10
};
\legend{};
\end{axis}


% \end{groupplot}

\end{tikzpicture}

